TAP-CAM: A Tunable Approximate Matching Engine based on Ferroelectric Content Addressable Memory

Pattern search is crucial in numerous analytic applications for retrieving data entries akin to the query. Content Addressable Memories (CAMs), an in-memory computing fabric, directly compare input queries with stored entries through embedded comparison logic, facilitating fast parallel pattern search in memory. While conventional CAM designs offer exact match functionality, they are inadequate for meeting the approximate search needs of emerging data-intensive applications. Some recent CAM designs propose approximate matching functions, but they face limitations such as excessively large cell area or the inability to precisely control the degree of approximation. In this paper, we propose TAP-CAM, a novel ferroelectric field effect transistor (FeFET) based ternary CAM (TCAM) capable of both exact and tunable approximate matching. TAP-CAM employs a compact 2FeFET-2R cell structure as the entry storage unit, and similarities in Hamming distances between input queries and stored entries are measured using an evaluation transistor associated with the matchline of CAM array. The operation, robustness and performance of the proposed design at array level have been discussed and evaluated, respectively. We conduct a case study of K-nearest neighbor (KNN) search to benchmark the proposed TAP-CAM at application level. Results demonstrate that compared to 16T CMOS CAM with exact match functionality, TAP-CAM achieves a 16.95x energy improvement, along with a 3.06% accuracy enhancement. Compared to 2FeFET TCAM with approximate match functionality, TAP-CAM achieves a 6.78x energy improvement.

==> 05_multibit.tex <==
%figure not finished yet


%\section{Multi-bit COSIME Implementation}

%\label{sec:multi-bit}
%{\color{red}So far, we've introduced vectors with binary values - '0' and '1'. However, application such as convolution neural network (CNN) that is mapped into vectors normally is presented in several weights rather than simply zeros and ones.
%Recent work for in-memory multi-bit multiplication approaches the canonical SRAM along with analog operations, the work uses either traditional 6T SRAMs in~\cite{sujan2018,IMAC,bitline_shifting}, or less-area efficient 8T or 10T cells for in-memory multi-bit multiplication~\cite{8T,biswas2018conv}. Besides, a fully-digital standard-cell-based CMOS in-memory multi-bit multiplication is presented in \cite{PPAC}.
%However, the peripherals in these works are complex as they introduce successive approximation analog-to-digital converter (SAR-ADC) and other digital peripherals, leading to higher search delay, and the conventional SRAM itself isn't area-efficient enough.

%Here, we propose an area and energy efficient way of analog-like in-memory multiplication. Similar to \cite{8T}, it's necessary to operate the input MOSFET of a cell in a particular voltage range such that the current is a linear function of the applied voltage $V_{in}$. But unlike prior work leveraging conventional SRAM, we make use of the same 1F1R structure as the binary {\cosi} discussed in \ref{sec:mem_array}, and a MOSFET that operates in the deep triode region (Eq.~\ref{eq:triode}) to serve as the input.
%\subsection{Schematic of 4-bit Cell}
%Let us consider a 4-bit precision for the weights. If the weight $W = w_3w_2w_1w_0$, where $w_i,i=0\sim 3$ corresponding to the 4-bit weight, the vector matrix dot product becomes:
% \begin{equation}\label{eq:4bit}
% \small
%     \begin{aligned}
%         &\sum(v_{in}\cdot W) = \sum[v_{in}\cdot(2^3w_3+2^2w_2+2^1w_1+2^0w_0)]\\
%         &=\sum(v_{in}\cdot2^3w_3)+\sum(v_{in}\cdot2^2w_2)+\sum(v_{in}\cdot2^1w_1)+\sum(v_{in}\cdot2^0w_0)
%     \end{aligned}
% \end{equation}
%Let us consider a cell with 4-bit weight $W = w_3w_2w_1w_0$. With a 4-bit input $V_{in}$, the output current should satisfy the following equation:
%\begin{equation}\label{eq:4bit}
%        I = V_{in} \cdot W = V_{in} \cdot (2^3w_3+2^2w_2+2^1w_1+2^0w_0)
%\end{equation}
%In {\cosi}, the weight, i.e. $2^3:2^2:2^1:2^0$, is achieved by the resistor applied in each 1F1R structure. The binary bits in Eq.~\ref{eq:4bit}, i.e. $w_3\sim w_0$, are stored in the FeFET in each 1F1R structure respectively. Finally, the input voltage $V_{in}$ is inputted through a MOSFET that operates in deep triode region. The $I_{DS}$ flows through a MOSFET/FeFET that operates in deep triode region can be characterized as follows:
%\begin{equation}\label{eq:triode}
%    \begin{aligned}
%    I_{DS} = \frac{\mu C_{ox}}{2}&\frac{W}{L}[2(V_{GS}-V_{TH})V_{DS}-V_{DS}^2],\\ &\text{with} V_{GS}>V_{TH}, V_{DS}<V_{GS}-V_{TH}
%    \end{aligned}
%\end{equation}
%where $\mu$ is the mobility of electrons, $C_{ox}$ is the silicon oxide, and $V_{TH}$ is the threshold voltage. In COSIME, the quadratic $V_{DS}$ term can be ignore since the operating current is small due to the large resistor applied in 1F1R structure. The MOSFET that serves as an input should operate in deep triode region, once it enters saturation, the multiplication can no longer be performed (see Fig.~\ref{fig:all}).

%In short, the stored value in multi-bit {\cosi} is binary, while the input value can be selected from 0 to 1.2V, depending on the weight of the input value, and for voltage that is higher than 1.2V, since the input MOSFET enters saturation, the mapping will be the same as 15. 



%\subsection{Experimental setup of Multi-bit Cell}

%In our SPICE experimental setup, each FeFETs is first programmed to either high/low-$V_{TH}$ state with 100ns $\pm4V$ pulse, as stated in Sec.~\ref{sec:background}. Then, the gate voltage of each FeFETs, $V[3]\sim V[0]$, is simply set to '1' (see Fig.~\ref{fig:cell_wave}(a)). Consequently, if the stored value in FeFET is zero, the output current $I_D$ of that certain 1F1R will be '0', on the contrary, will be '1'. With the proposed 1F1R structure, the ratio of the $I_D$ flows through each 1F1Rs' rails in a cell can reach 8:4:2:1. In {\cosi}, $R_0=2.5\times 10^8$, $R_1=1.25\times 10^8$, $R_2=0.625\times 10^8$, and $R_3=0.3125\times 10^8$ (see Fig.~\ref{fig:cell_wave}). The input MOSFET will be activated during the search. In Fig.~\ref{fig:cell_wave}(a), the 4-bit input is mapped into 16 different voltages.

%\subsection{Multi-function Crossbar COSIME}
%To this end, we proposed a dedicated in-memory search engine for cosine similarity. However, practical applications usually involve various functions~\cite{ReFeMAT}. To make {\cosi} supports other well-studied functions such as Hamming distance/binary convolution neural network (BCNN), another 1F1R is added on the basis of Fig.~\ref{fig:cell_wave}, which can be seen in Fig.~\ref{fig:cell}.
%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{Figures/new-multi-bit-cell.png}
%    \caption{{\color{red}{\cosi} cell supports Hamming distance and multi-bit multiplication on the basis of Fig.~\ref{fig:cell_wave}(a). The orange background color supports multi-bit multiplication while the green square supports Hamming distance.}}
%    \label{fig:cell}
%\end{figure}
%To support both multi-bit in-memory multiplication and Hamming distance, the crossbar array for the denominator of translinear circuit input, i.e. the $I_y$ in Eq.~\ref{eq:translinear}, is simply set to a constant. In multi-bit multiplication mode, the gate voltage of FeFET, i.e. $V[3]\sim V[0]$, is set to '1' when the query vector comes (see the waveform in Fig.~\ref{fig:cell_wave}). On the other hand, when {\cosi} operates in Hamming distance mode, $V[3]\sim V[1]$ will simply be set to '0' when the query comes.
%Consequently, {\cosi} consumes less search energy while functioning in these mode.
%}



==> 08_Biography.tex <==
% \begin{IEEEbiographynophoto}{Che-Kai Liu}
% is currently working toward B.Eng. degree with the College of Information Science and Electronic Engineering, Zhejiang University, China. He is also an undergraduate researcher at Zhejiang University and University of Notre Dame, USA, working with Dr. Xunzhao Yin and Dr. X. Sharon Hu, respectively. His research interests include brain-inspired computing and novel computing paradigms with both CMOS
% and emerging technologies.
% \end{IEEEbiographynophoto}

% \begin{IEEEbiographynophoto}{Haobang Chen}
% is currently a junior at Zhejiang University, Hangzhou, China. He  is working towards a B.Eng. degree of Electronics Science and Technology. His current research interests focus on Computation-in-Memory
% architectures and machine learning.

% \end{IEEEbiographynophoto}

% \begin{IEEEbiographynophoto}{Mohsen Imani}
% (S’14) received the B.Sc. and M.S. degrees from the School of Electrical and Computer Engineering, University of Tehran, Tehran, Iran, in 2011 and 2014, respectively, and the Ph.D. degree with the Department of Computer Science and Engineering, University of California at San Diego, La Jolla, CA, USA, in 2020. He is now an Assistant Professor with the University of California, Irvine. His current research interests include brain-inspired computing, approximation computing, and processing in-memory architectures.
% \end{IEEEbiographynophoto}

% \begin{IEEEbiographynophoto}{Kai Ni}
% received the B.S. degree in Electrical Engineering from University of Science and Technology of China, Hefei, China in 2011, and Ph.D. degree of Electrical Engineering from Vanderbilt University, Nashville, TN, USA in 2016 by working on characterization, modeling, and reliability of III-V MOSFETs. Since then, he became a postdoctoral associate at University of Notre Dame, working on ferroelectric devices for nonvolatile memory and novel computing paradigms. He is now an assistant professor in Electrical and Microelectronic Engineering at Rochester Institute of Technology. He has 80 publications in top journals and conference proceedings, including Nature Electronics, IEDM, VLSI Symposium, IRPS, EDL, etc. His current interests lie in nanoelectronic devices empowering unconventional computing, AI accelerator, 3D memory technology.
% \end{IEEEbiographynophoto}

% \begin{IEEEbiographynophoto}{Arman Kazemi}
% is a Ph. D. candidate at the University of Notre Dame and is co-advised by Dr. X. Sharon Hu and Dr. Michael Niemier. His research interests include hardware/software co-design, low-power hardware design, and in-memory computing. He is particularly interested in inventions leveraging emerging beyond-CMOS technologies e.g. ferroelectric materials. His research usually targets reducing computational resource requirements of machine learning applications using emerging circuits and architectures. He has been nominated for the best paper award at DATE 2021.
% \end{IEEEbiographynophoto}

% \begin{IEEEbiographynophoto}{Ann Franchesca Laguna}
% received her MS degree in Electrical Engineering and BS degree in Computer Engineering from University of the Philippines – Diliman. She is currently a Computer Science and Engineering PhD student at University of Notre Dame working with Dr. X. Sharon Hu and Dr. Michael Niemier. Her current research interests encompass hardware/software co-design of machine learning and bioinformatics algorithms using in-memory computing.
% \end{IEEEbiographynophoto}

% \begin{IEEEbiographynophoto}{Michael Niemier}
% (senior member, IEEE) is a Professor at the University of Notre Dame. His research interests include designing, benchmarking, and evaluating circuits and architectures based on emerging technologies. Currently, Niemier's research efforts are based on new transistor technologies, as well as devices based on alternative state variables such as spin. He is the recipient of an IBM Faculty Award, the Rev. Edmund P. Joyce, C.S.C. Award for Excellence in Undergraduate Teaching at the University of Notre Dame, as well as the Department of Computer Science and Engineering Teaching Award at the University of Notre Dame. Niemier has served on numerous technical program committees for design-related conferences (including DAC, DATE, ICCAD, etc.), and has chaired the emerging technologies track at DATE, DAC, and ICCAD. He is an associated editor for IEEE Transactions on Nanotechnology, as well as the ACM Journal of Emerging Technologies in Computing.
% \end{IEEEbiographynophoto}

% \begin{IEEEbiographynophoto}{Xiaobo Sharon Hu}
% (Fellow, IEEE) received a BS degree from Tianjin University, in 1982, an MS degree from the Polytechnic Institute of New York, in 1984, and a Ph.D. degree from Purdue University, in 1989. She is currently a professor with the Department of Computer Science and Engineering, University of Notre Dame. Her research interests include computing with beyond-CMOS technologies, low-power system design, and cyber-physical systems. She received the NSF CAREER Award in 1997, and the Best Paper Award from the DAC, in 2001, and the ACM/IEEE International Symposium on Low Power Electronics and Design, in 2018. She was the general chair of DAC'18. She served as an associate editor of the IEEE Transactions on VLSI Systems, ACM Transactions on Design Automation of Electronic Systems, and ACM Transactions on Embedded Computing. She is currently an associate editor of the ACM Transactions on Cyber-Physical Systems.
% \end{IEEEbiographynophoto}

% \begin{IEEEbiographynophoto}{Liang Zhao} is a tenure-track research professor with the College of Information Science and Electronic Engineering at Zhejiang University. He received his Ph.D. degree in Electrical Engineering from Stanford University in 2015 and B.S. degree in Microelectronics from Tsinghua University in 2010, respectively. His research interests include emerging non-volatile memories, semiconductor device modeling and simulations, as well as circuits and architectures for neuromorphic computing. He has received the best student paper award of VLSI-TSA 2014 and the best student paper nomination of VLSI Symposia 2013. He is a member of IEEE.
% \end{IEEEbiographynophoto}

% \begin{IEEEbiographynophoto}{Cheng Zhuo}
% (S’06-M’12-SM’16) received the B.S. and M.S. degrees from Zhejiang University, China, in 2005 and 2007, respectively, and the Ph.D. degree in computer science and engineering from the University of Michigan, Ann Arbor, MI, in 2010. He is currently a Professor with the College of Information Science Electronic Engineering, Zhejiang University. His research interests include low power optimization, 3-D integration, hardware acceleration, power and signal integrity. Dr. Zhuo has published over 100 technical papers and received 4 Best Paper Nominations in DAC'16, CSTIC'18, ICCAD'20, and VTS'21. He also received 2012 ACM SIGDA Technical Leadership Award and 2017 JSPS Invitation Fellowship. Dr. Zhuo has served on the technical program and organization committees of many international conferences, and as the Associate Editors of IEEE TCAD, ACM TODAES, and Elsevier {Integration}. He is a senior member of IEEE and a Fellow of IET.
% \end{IEEEbiographynophoto}

% \begin{IEEEbiographynophoto}{Xunzhao Yin}(S'16-M'19) is an assistant professor of the College of Information Science and Electronic Engineering at Zhejiang University. He received his Ph.D. degree in Computer Science and Engineering from University of Notre Dame in 2019 and B.S. degree in Electronic Engineering from Tsinghua University in 2013, respectively. His research interests include emerging circuit/architecture designs and novel computing paradigms with both CMOS and emerging technologies. He has received the best paper award nomination of ICCAD 2020, the Outstanding Research Assistant Award in the department of CSE at University of Notre Dame in 2017, and Bronze medal of Student Research Competition at ICCAD 2016, etc. He is a member of IEEE.
% \end{IEEEbiographynophoto}
